A Game Characterization for Contrasimilarity

We present the first game characterization of contrasimilarity, the weakest form of bisimilarity. The game is finite for finite-state processes and can thus be used for contrasimulation equivalence checking, of which no tool has been capable to date. A machine-checked Isabelle/HOL formalization backs our work and enables further use of contrasimilarity in verification contexts.

==> eptcsdata.tex <==
\providecommand{\firstpage}{27}
\providecommand{\publicationstatus}{V. Castiglioni and O. Dardha (Eds.): Combined Workshop on \\Expressiveness in Concurrency and Structural Operational Semantics \\ (EXPRESS/SOS 2021)\\
EPTCS 339, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.339.5}{10.4204/EPTCS.339.5}}
\pdfoutput=1

